EffiBench-X: A Multi-Language Benchmark for Measuring Efficiency of LLM-Generated Code

Existing code generation benchmarks primarily evaluate functional correctness, with limited focus on code efficiency and often restricted to a single language like Python. To address this gap, we introduce EffiBench-X, the first multi-language benchmark designed to measure the efficiency of LLM-generated code. EffiBench-X supports Python, C++, Java, JavaScript, Ruby, and Golang. It comprises competitive programming tasks with human-expert solutions as efficiency baselines. Evaluating state-of-the-art LLMs on EffiBench-X reveals that while models generate functionally correct code, they consistently underperform human experts in efficiency. Even the most efficient LLM-generated solutions (Qwen3-32B) achieve only around \textbf{62\%} of human efficiency on average, with significant language-specific variations. LLMs show better efficiency in Python, Ruby, and JavaScript than in Java, C++, and Golang. For instance, DeepSeek-R1's Python code is significantly more efficient than its Java code. These results highlight the critical need for research into LLM optimization techniques to improve code efficiency across diverse languages. The dataset and evaluation infrastructure are submitted and available at https://github.com/EffiBench/EffiBench-X.git and https://huggingface.co/datasets/EffiBench/effibench-x.

==> case_study/best_case_1/potential_description.tex <==
In this best-case comparison, we observe that both the \textbf{DeepSeek-Reasoner}-generated code and the canonical solution follow a \textbf{greedy approach}: always perform the most expensive remaining cut first. This is a classic greedy cut-cost minimization problem that benefits from sorting and piece-count tracking.

Both implementations:
\begin{itemize}
    \item Sort the cut costs in descending order,
    \item Track how many horizontal and vertical pieces exist,
    \item Multiply the cost of the cut by the number of affected pieces.
\end{itemize}

The key similarity lies in recognizing that the cost of each cut grows linearly with the number of pieces it intersects. The alignment in logic and structure leads to a nearly identical runtime, demonstrating that LLMs can naturally synthesize optimal greedy solutions.



==> case_study/best_case_2/potential_description.tex <==
This illustrates a best-case scenario where the solution generated by \texttt{DeepSeek-Reasoner} closely matches the human-written canonical solution, both in structure and runtime efficiency (ratio = 0.985). The problem requires computing the sum of absolute differences between adjacent characters' ASCII values in a given string. 

The \texttt{DeepSeek-Reasoner} implementation uses a forward loop from index 1, calculating \texttt{abs(ord(s[i]) - ord(s[i-1]))}, while the canonical solution performs the same calculation from index 0 using \texttt{abs(ord(s[i]) - ord(s[i+1]))}. These two approaches are functionally equivalent due to the symmetric nature of the absolute difference, and both operate in linear time complexity $\mathcal{O}(n)$ with constant space usage. 

This convergence highlights the LLM's ability to infer optimal solutions not only from the problem description but also from general coding patterns. Unlike worst-case examples where LLMs diverge in algorithm design or introduce unnecessary overhead, this case demonstrates a high-quality, generalized solution that mirrors expert-level efficiency and readability.


==> case_study/best_case_3/potential_description.tex <==
This figure illustrates a best-case example in which the code generated by Claude-3.7-Sonnet almost perfectly replicates the canonical solution. The task is to return the XOR of all numbers that appear exactly twice in an array. Both implementations adopt the same high-level strategy:

\begin{itemize}
  \item Count the frequency of each element in the input array.
  \item Iterate through the frequency map and apply the XOR operation only to elements with a frequency of two.
\end{itemize}

The canonical solution employs a \texttt{map}, which maintains ordering but results in slightly higher overhead due to its \texttt{O(log N)} access and insertion times. In contrast, the LLM-generated code optimizes performance by utilizing an \texttt{unordered\_map}, which allows for average-case \texttt{O(1)} access and insertion, demonstrating not only correctness but also superior performance awareness.

This case exemplifies a high-efficiency general solution, where the LLM demonstrates an understanding of optimal data structures and adheres to clean, human-like code organization. It highlights Claude's capability to generate competitive solutions that are not only correct but also efficient, often rivaling or even surpassing human-written implementations in specific scenarios.


==> case_study/worse_case_1/potential_description.tex <==
\subsection{Case Study: Inefficient Dynamic Programming in \texttt{String Contains 'leet'} Task}

The solution generated by \textbf{Claude-3.7-Sonnet} for counting the number of good strings, which can be rearranged to contain \texttt{"leet"} as a substring, exemplifies a clear inefficiency in both memory and runtime performance. The task requires counting strings of length $n$ that contain at least one character \texttt{l}, at least two \texttt{e}'s, and one \texttt{t}.

Claude-3.7-Sonnet approaches this problem using a 4-dimensional dynamic programming (DP) table. Specifically, the state \texttt{dp[i][l][e][t]} records the number of strings of length $i$ with $l$ occurrences of \texttt{l}, $e$ of \texttt{e}, and $t$ of \texttt{t}, capped respectively at $1$, $2$, and $1$. This results in a state space of size $O(n \times 2 \times 3 \times 2)$, and the model updates each state at every iteration. While the solution is logically correct, it suffers from redundant state expansions and excessive memory usage, especially for large $n$. The model does not employ pruning strategies, prefix-counting optimizations, or algebraic transformations, and instead falls back on a simulation-based enumeration of state transitions.

In contrast, the \textbf{canonical solution} adopts a concise and efficient analytical approach using the \textit{Inclusion-Exclusion Principle}. Rather than enumerating each valid string, it directly subtracts the number of invalid strings (e.g., those missing required characters) from the total $26^n$. By leveraging combinatorial identities and fast modular exponentiation, it computes the final result in $O(\log n)$ time with constant space.

This example clearly illustrates a broader pattern observed in LLM-generated code: while often logically valid, such solutions tend to lack mathematical abstraction and optimization, opting instead for generic enumeration techniques. In this case, the Claude-3.7-Sonnet solution was approximately \textbf{33$\times$ slower} and significantly more memory-intensive than the canonical one, underscoring its limitations in recognizing mathematically structured problem-solving strategies.


==> case_study/worse_case_2/potential_description.tex <==
\paragraph{Case Study: Make $K$ Most Frequent}
We compare the performance between \texttt{Claude-3.7-Sonnet}'s generated solution and the human-written canonical implementation. The LLM-generated code performs an exhaustive $\mathcal{O}(n^2)$ search over all possible subarrays to determine the minimal number of operations required to make $K$ the most frequent element in the array. Although logically correct, this approach is computationally expensive and becomes inefficient on large inputs.

In contrast, the canonical solution adopts a linear-time strategy by considering only two types of boundary operations—prefix and suffix removal. It maintains frequency counters and efficiently checks whether removing a continuous segment from either end is sufficient to achieve the goal. This significantly reduces both the number of operations and memory overhead. Overall, this example illustrates that while LLMs are capable of understanding the problem intent, they often lack the algorithmic optimization required for efficient and scalable solutions.


==> sections/stat.tex <==
\section{Benchmark Statistics}
\label{sec:stats}

\input{tables/dataset_stat}
We provide detailed statistics of the dataset in \cref{tab:dataset}. 
The coding problems in \dataset have three difficulty levels (171 easy, 589 medium, and 240 hard), where the difficulty of each problem is defined by LeetCode \cite{LeetCode}. The table lists the number of problems for each algorithm.
Specifically, \dataset contains 243 problems for greedy algorithms, 277 for dynamic programming (DP), 48 for backtracking, 21 for divide and conquer, 108 for depth-first search (DFS), 86 for breadth-first search (BFS), 148 for binary search, 105 for two pointers, 70 for sliding window, 102 for bit manipulation, and 238 for sorting algorithms. 
The sum of problems across algorithm categories can exceed the total number of problems because one problem in our dataset may belong to multiple algorithm classes. On average, a problem description in \dataset contains 212.0 words. The canonical solutions, which represent the baseline code against which the generated code is compared, have 14.6 lines on average. 

\cref{tab:dataset_comparison} compares \dataset with five widely used code datasets (HumanEval, MBPP, APPS, DSP, DS-1000). Unlike prior datasets focused primarily on pass rates, \dataset also analyzes efficiency during execution. 
Although \dataset is primarily designed to assess the efficiency of generated code, it can also be used to evaluate code correctness, akin to other code generation datasets. 


